Windowed space-time least-squares Petrov-Galerkin method for nonlinear model order reduction

This work presents the windowed space-time least-squares Petrov-Galerkin method (WST-LSPG) for model reduction of nonlinear parameterized dynamical systems. WST-LSPG is a generalization of the space-time least-squares Petrov-Galerkin method (ST-LSPG). The main drawback of ST-LSPG is that it requires solving a dense space-time system with a space-time basis that is calculated over the entire global time domain, which can be unfeasible for large-scale applications. Instead of using a temporally-global space-time trial subspace and minimizing the discrete-in-time full-order model (FOM) residual over an entire time domain, the proposed WST-LSPG approach addresses this weakness by (1) dividing the time simulation into time windows, (2) devising a unique low-dimensional space-time trial subspace for each window, and (3) minimizing the discrete-in-time space-time residual of the dynamical system over each window. This formulation yields a problem with coupling confined within each window, but sequential across the windows. To enable high-fidelity trial subspaces characterized by a relatively minimal number of basis vectors, this work proposes constructing space-time bases using tensor decompositions for each window. WST-LSPG is equipped with hyper-reduction techniques to further reduce the computational cost. Numerical experiments for the one-dimensional Burgers' equation and the two-dimensional compressible Navier-Stokes equations for flow over a NACA 0012 airfoil demonstrate that WST-LSPG is superior to ST-LSPG in terms of accuracy and computational gain.

==> commands.tex <==
\numberwithin{equation}{section}


\newlist{Assumption}{enumerate}{1}
\setlist[Assumption]{label=A\arabic*}

\makeatletter


\newcommand{\multiline}[1]{%
  \begin{tabularx}{\dimexpr\linewidth-\ALG@thistlm}[t]{@{}X@{}}
    #1
  \end{tabularx}
}

\newcommand{\thickhline}{%
    \noalign {\ifnum 0=`}\fi \hrule height 1pt
    \futurelet \reserved@a \@xhline
}


\newcommand*\MY@leftharpoonupfill@{%
    \arrowfill@\leftharpoonup\relbar\relbar
}
\newcommand*\MY@rightharpoonupfill@{%
    \arrowfill@\relbar\relbar\rightharpoonup
}
\newcommand*\MY@rightarrowfill@{%
    \arrowfill@\relbar\relbar\rightarrow
}
\newcommand*\MY@rightapproxupfill@{%
    \arrowfill@\relbar\relbar\appro
}
\newcommand*\overleftharpoon{%
    \mathpalette{\overarrow@\MY@leftharpoonupfill@}%
}
\newcommand*\overrightharpoon{%
    \mathpalette{\overarrow@\MY@rightharpoonupfill@}%
}
\newcommand*\overrightapprox{%
    \mathpalette{\overarrow@\MY@rightapproxupfill@}%
}
\makeatother
% \newcommand{\harpoon}{\overset{\rightharpoonup}}

% Enable two line label
% I added \RaggedRight from the `ragged2e' package here to avoid
% over- and underfull boxes
% \renewcommand{\nomlabel}[1]{%
%   \smash{\parbox[t]{.05\linewidth}{\RaggedRight#1}}}
  
% \renewcommand{\nomgroup}[1]{%
%   \ifx#1U\relax
%     \item[\grouphead{States}]
%   \fi
%   \ifx#1R\relax
%     \item[\grouphead{Residuals}]
%   \fi
%   \ifx#1W\relax
%     \item[\grouphead{Dummy Variables}]
%   \fi
%   \ifx#1X\relax
%     \item[\grouphead{Tensors/Snapshots}]
%   \fi
%   \ifx#1S\relax
%     \item[\grouphead{Subspaces}]
%   \fi
%   \bigskip}
  
% \usepackage{amsmath,scalerel}
% \newcommand\doverline[1]{\ThisStyle{%
%   \setbox0=\hbox{$\SavedStyle\widetilde{#1}$}%
%   \ht0=\dimexpr\ht0-.25ex\relax% CHANGE .15 TO AFFECT SPACING
%   \overrightharpoon{\copy0}%
% }}

% \definecolor{Blue}{rgb}{0,0,1}
% \definecolor{Red}{rgb}{1,0,0}
% \definecolor{Green}{rgb}{0,1,0}

\stackMath
\newcommand\goodhat[1]{%
\savestack{\tmpbox}{\stretchto{%
  \scaleto{%
    \scalerel*[\widthof{\ensuremath{#1}}]{\kern.8pt\mathchar"0362\kern.1pt}%
    {\rule{0ex}{\textheight}}%WIDTH-LIMITED CIRCUMFLEX
  }{\textheight}% 
}{2.4ex}}%
\stackon[-6.9pt]{#1}{\tmpbox}%
}
\parskip 1ex


%\newcommand{\snaps}[1]{\ensuremath{\snapsNo_{#1}}}  % timestep at optional
\newcommand{\KTC}[1]{{\textcolor{Blue}{KTC: #1}}}
%\newcommand{\CH}[1]{{\textcolor{Red}{CH: #1}}}
\newcommand{\YC}[1]{{\textcolor{Blue}{YC: #1}}}
\newcommand{\YS}[1]{{{\color{blue}{YS: #1}}}}
\newcommand{\EP}[1]{{{\color{red}{EP: #1}}}}
\newcommand{\EPCR}[2]{{\color{red}\st{#1}{#2}}}
\newcommand{\EPC}[1]{{\color{red}\st{#1}}}
%\newcommand{\reviewerA}[1]{{\color{blue}{#1}}}
%\newcommand{\reviewerB}[1]{{\color{red}{#1}}}
%\newcommand{\reviewerBRtwo}[1]{{\color{red}{#1}}}
%\newcommand{\ourReReading}[1]{{\color{violet}{#1}}}
\newcommand{\reviewerA}[1]{#1}
\newcommand{\reviewerB}[1]{#1}
\newcommand{\reviewerBRtwo}[1]{#1}
%\newcommand{\reviewerBRthree}[1]{{\color{red}{#1}}}
\newcommand{\reviewerBRthree}[1]{#1}
\newcommand{\ourReReading}[1]{#1}
\newcommand{\fontContinuousFunc}{ \mathcal}
\newcommand{\fontDiscreteFunc}{\mathscr}
\newcommand{\fontDiscrete}{\mathcal}
\newcommand{\knWindowArg}[2]{k^{#1,#2}}
\newcommand{\knArg}[1]{k(t^{#1})}
\newcommand{\kn}{\knArg{n}}
\newcommand{\knDummy}{k(\timeDummy^n)}
\newcommand{\kmax}{k_\text{max}}
\newcommand{\bds}[1]{{\boldsymbol{#1}}}
\newcommand{\highlight}[1]{{\textcolor{Red}{#1}}}
\newcommand{\defeq}{:=}
\newcommand{\eqdef}{=:}
\newcommand{\SPSD}[1]{\text{SPSD}(#1)}
\newcommand{\optDummy}{v}
\newcommand{\orthomat}[2]{\mathbb V_{{#2}}(\RR{{#1}})}
\newcommand{\domain}{\Omega}
\newcommand{\domaini}{\domain_i}
\newcommand{\boundary}{\Gamma}
\newcommand{\mappingNo}{\mathcal I}
\newcommand{\mapping}[2]{\mappingNo(#1,#2)}
\newcommand{\boundaryi}{\boundary_i}
\newcommand{\nsubdomains}{{n_\domain}}
\newcommand{\nconstraints}{n_{\bar A}}
\newcommand{\nconstraintsROM}{n_{A}}
\newcommand{\ninterfacedofs}{{n_\boundary}}
\newcommand{\residual}{\bds{r}}
\newcommand{\residualArg}[1]{\residual_{#1}}
\newcommand{\residuali}{\residualArg{i}}
\newcommand{\methodAcronym}{WST-LSPG}
\newcommand{\timeSpace}{\fontContinuousFunc T}
\newcommand{\timeDiscreteFuncSpace}{\mathcal{T}}
\newcommand{\timeDiscreteSpace}{\RR{\ntimedof}}
\newcommand{\spatialSpace}{\RR{\nspacedof}}
\newcommand{\unrollfunc}{\bds{g}}
% \newcommand{\vectorizeNone}{\vectorizefuncNo} % timestep at optional
% \newcommand{\vectorize}[1]{\ensuremath{\vectorizeNone(#1)}}  % timestep
% \newcommand{\vectorizeinv}[1]{\ensuremath{\vectorizeNone^{-1}(#1)}}  %
% \newcommand{\vectorizefuncNo}{\bds{h}}
% \newcommand{\vectorizefunc}[1]{{\vectorizefuncNo}(#1)}
\newcommand{\lipschitzK}{L_{\res}}
\newcommand{\inverseLipschitzK}{K_{\res}}
\newcommand{\lipschitzFK}{L_{\flux}}
\newcommand{\inverseLipschitzFK}{K_{\flux}}
\newcommand{\boundingConstantF}{M_{\flux}}
\newcommand{\arbitraryConstant}{C}
\newcommand{\abarConstant}{\kappa_1}
\newcommand{\aConstant}{\kappa_2}
\newcommand{\stbasisvecSubWindowEndTimeArg}[2]{{\boldsymbol \pi}_{#1}^{#2} }

\newcommand{\stateContinuousDummyEntryNo}{\boldsymbol{y}}
\newcommand{\stateContinuousDummyEntry}[1]{\stateContinuousDummyEntryNo_{#1}}
\newcommand{\stateContinuousDummy}[1]{\bds{\stateContinuousDummyEntryNo}} 
\newcommand{\stateTwoContinuousDummyEntryNo}{\boldsymbol{v}}
\newcommand{\stateTwoContinuousDummyEntry}[1]{\stateTwoContinuousDummyEntryNo_{#1}}
\newcommand{\stateTwoContinuousDummy}[1]{\bds{\stateTwoContinuousDummyEntryNo}} 
\newcommand{\metric}{\bds{\Theta}} 

\newcommand{\crossareaSymb}{A}
\newcommand{\externalforceSymb}{q}
\newcommand{\externalforce}{\boldsymbol \externalforceSymb}
\newcommand{\state}{\bds{u}}


\newcommand{\stateArg}[1]{\state^{#1}}
\newcommand{\statei}{\stateArg{i}}

\newcommand{\stateApprox}{\tilde\state}
\newcommand{\stateApproxArg}[1]{\stateApprox_{#1}}
\newcommand{\stateApproxi}{\stateApproxArg{i}}
\newcommand{\stateApproxInterior}{\tilde\state^\domain}
\newcommand{\stateApproxInteriorArg}[1]{\stateApproxInterior_{#1}}
\newcommand{\stateApproxInteriori}{\stateApproxInteriorArg{i}}
\newcommand{\stateApproxBoundary}{\tilde\state^\boundary}
\newcommand{\stateApproxBoundaryArg}[1]{\stateApproxBoundary_{#1}}
\newcommand{\stateApproxBoundaryi}{\stateApproxBoundaryArg{i}}

\newcommand{\stateInterior}{\bds{x}^{\Omega}}
\newcommand{\stateInteriorArg}[1]{\stateInterior_{#1}}
\newcommand{\stateInteriori}{\stateInteriorArg{i}}

\newcommand{\stateBoundary}{\bds{x}^{\Gamma}}
\newcommand{\stateBoundaryArg}[1]{\stateBoundary_{#1}}
\newcommand{\stateBoundaryi}{\stateBoundaryArg{i}}

\newcommand{\projection}{\bds{P}}
\newcommand{\projectionRes}{\projection^\residual}
\newcommand{\projectionResArg}[1]{\projectionRes_{#1}}
\newcommand{\projectionResi}{\projectionResArg{i}}
\newcommand{\jacobianST}[2]{{\boldsymbol J_{#1,#2}}}
\newcommand{\jacobianWST}[3]{{\boldsymbol J_{#1,#2}^{#3}}}

\newcommand{\projectionStateInterior}{\projection^\Omega}
\newcommand{\projectionStateInteriorArg}[1]{\projectionStateInterior_{#1}}
\newcommand{\projectionStateInteriori}{\projectionStateInteriorArg{i}}

\newcommand{\projectionStateBoundary}{\bds{P}^\Gamma}
\newcommand{\projectionStateBoundaryArg}[1]{\projectionStateBoundary_{#1}}
\newcommand{\projectionStateBoundaryi}{\projectionStateBoundaryArg{i}}


\newcommand{\rbGlobal}{\bds{\Phi}}
\newcommand{\rbBubble}{\bds{\Phi}^\domain}
\newcommand{\rbBubbleArg}[1]{\rbBubble_{#1}}
\newcommand{\rbBubblei}{\rbBubbleArg{i}}
\newcommand{\rbBoundary}{\bds{\Phi}^\boundary}
\newcommand{\rbBoundaryArg}[1]{\rbBoundary_{#1}}
\newcommand{\rbBoundaryi}{\rbBoundaryArg{i}}
\newcommand{\rbInterior}{\bds{\Phi}^\domain}
\newcommand{\rbInteriorArg}[1]{\rbInterior_{#1}}
\newcommand{\rbInteriori}{\rbInteriorArg{i}}
\newcommand{\rbPort}{\bds{\Phi}^p}
\newcommand{\rbPortArg}[1]{\rbPort_{#1}}
\newcommand{\rbPorti}{\rbPortArg{i}}
\newcommand{\rbPortj}{\rbPortArg{j}}
\newcommand{\rbInterface}{\bds{\Phi}^y}

\newcommand{\redState}{\hat {\bds x}}
\newcommand{\redStateArg}[1]{\redState_{#1}}
\newcommand{\redStateBoundary}{\redState^\boundary}
\newcommand{\redStateBoundaryArg}[1]{\redStateBoundary_{#1}}
\newcommand{\redStateBoundaryi}{\redStateBoundaryArg{i}}
\newcommand{\redStateBoundaryisol}{\redStateBoundaryArg{i\star}}
\newcommand{\redStateBoundaryNullVar}{\bds{y}}
\newcommand{\redStateBoundaryNull}{\redStateBoundaryNullVar^\boundary}

\newcommand{\redStateInterface}{\hat{\bds{y}}}

\newcommand{\redStateInterior}{\redState^\domain}
\newcommand{\redStateInteriorArg}[1]{\redStateInterior_{#1}}
\newcommand{\redStateInteriori}{\redStateInteriorArg{i}}
\newcommand{\redStateInteriorisol}{\redStateInteriorArg{i\star}}


%dimensions
\newcommand{\ndof}{\nspacedof}
\newcommand{\ndofi}{n_i}
\newcommand{\ndofInteriori}{n^{\Omega}_i}
\newcommand{\ndofBoundaryi}{n^{\Gamma}_i}
\newcommand{\nresi}{n^\residual_i}
\newcommand{\weightmatRows}{z}
\newcommand{\weightmatRowsArg}[1]{\weightmatRows^{#1}}
\newcommand{\weightmatRowsn}{\weightmatRowsArg{n}}
\newcommand{\weightmatstRows}{\bar z}
\newcommand{\weightmatstRowsArg}[1]{\weightmatstRows^{#1}}
\newcommand{\weightmatstRowsn}{\weightmatstRowsArg{n}}

\newcommand{\weightmatwstRowsArg}[1]{\weightmatstRows^{#1}}

\newcommand{\nrb}{p}
\newcommand{\nrbInterior}{\nrb^\domain}
\newcommand{\nrbInteriorArg}[1]{\nrbInterior_{#1}}
\newcommand{\nrbInteriori}{\nrbInteriorArg{i}}
\newcommand{\nrbBoundary}{\nrb^\boundary}
\newcommand{\nrbBoundaryArg}[1]{\nrbBoundary_{#1}}
\newcommand{\nrbBoundaryi}{\nrbBoundaryArg{i}}
\newcommand{\nrbPort}{\nrb^p}
\newcommand{\nrbPortArg}[1]{\nrbPort_{#1}}
\newcommand{\nrbPorti}{\nrbPortArg{i}}
\newcommand{\nrbPortj}{\nrbPortArg{j}}
\newcommand{\nrbInterface}{\nrb^y}


\newcommand{\constraintMat}{\bds{\bar A}}
\newcommand{\constraintMatArg}[1]{\constraintMat_{#1}}
\newcommand{\constraintMati}{\constraintMatArg{i}}
\newcommand{\constraintMatROM}{\bds{A}}
\newcommand{\constraintMatROMArg}[1]{\constraintMatROM_{#1}}
\newcommand{\constraintMatROMi}{\constraintMatROMArg{i}}

\newcommand{\hessianIntInt}{\bds{H}^{\domain\domain}}
\newcommand{\hessianIntIntArg}[1]{\hessianIntInt_{#1}}
\newcommand{\hessianIntInti}{\hessianIntIntArg{i}}


\newcommand{\hessianIntBound}{\bds{H}^{\domain\boundary}}
\newcommand{\hessianIntBoundArg}[1]{\hessianIntBound_{#1}}
\newcommand{\hessianIntBoundi}{\hessianIntBoundArg{i}}

\newcommand{\hessianBoundInt}{\bds{H}^{\boundary\domain}}
\newcommand{\hessianBoundIntArg}[1]{\hessianBoundInt_{#1}}
\newcommand{\hessianBoundInti}{\hessianBoundIntArg{i}}

\newcommand{\hessianBoundBound}{\bds{H}^{\boundary\boundary}}
\newcommand{\hessianBoundBoundArg}[1]{\hessianBoundBound_{#1}}
\newcommand{\hessianBoundBoundi}{\hessianBoundBoundArg{i}}

\newcommand{\searchDirInterior}{\bds{p}^\domain}
\newcommand{\searchDirInteriorArg}[1]{\searchDirInterior_{#1}}
\newcommand{\searchDirInteriori}{\searchDirInteriorArg{i}}

\newcommand{\searchDirLagrange}{\bds{p}^\lagrange}
\newcommand{\searchDirInterface}{\bds{p}^\redStateBoundaryNullVar}

\newcommand{\searchDirBoundary}{\bds{p}^\boundary}
\newcommand{\searchDirBoundaryArg}[1]{\searchDirBoundary_{#1}}
\newcommand{\searchDirBoundaryi}{\searchDirBoundaryArg{i}}

\newcommand{\redResState}{\hat{\bds{r}}_\bds{x}}
\newcommand{\redResLagrange}{\hat{\bds{r}}_\lagrange}

\newcommand{\redResBoundary}{\hat{\bds{r}}^\boundary}
\newcommand{\redResBoundaryArg}[1]{\redResBoundary_{#1}}
\newcommand{\redResBoundaryi}{\redResBoundaryArg{i}}

\newcommand{\redResInterior}{\hat{\bds{r}}^\domain}
\newcommand{\redResInteriorArg}[1]{\redResInterior_{#1}}
\newcommand{\redResInteriori}{\redResInteriorArg{i}}

\newcommand{\dualProblem}{h}
\newcommand{\dualProblemArg}[1]{\dualProblem_{#1}}
\newcommand{\dualProblemi}{\dualProblemArg{i}}

\newcommand{\unitvec}{\bds{e}}
\newcommand{\unitvecArg}[1]{\unitvec_{#1}}
\newcommand{\spacetimeindexNo}{\varphi}
\newcommand{\spacetimeindex}[2]{\varphi(#1,#2)}
\newcommand{\spacetimeindexIncludeAll}[1]{\spacetimeindex{\spaceindex{#1}}{\timeindex{#1}}}
\newcommand{\spacetimeindexIncludeAllSmall}[1]{\spacetimeindex{\spaceindexsmall{#1}}{\timeindexsmall{#1}}}
\newcommand{\spaceindexNo}{\mathcal s}
\newcommand{\timeindexNo}{\mathcal t}
\newcommand{\spaceindex}[1]{\mathcal s_{#1}}
\newcommand{\timeindex}[1]{\mathcal t_{#1}}
\newcommand{\spaceindexsmall}[1]{\mathcal s_{#1}'}
\newcommand{\timeindexsmall}[1]{\mathcal t_{#1}'}
\newcommand{\spacetimesampleset}{\mathfrak{st}}
\newcommand{\spacetimesamplesetsmall}{\spacetimesampleset'}
\newcommand{\samplematstsmall}{\samplematst'}

\newcommand{\resIndexSet}{I}
\newcommand{\resIndexSetArg}[1]{\resIndexSet_{#1}}
\newcommand{\resIndexSeti}{\resIndexSetArg{i}}

\newcommand{\nullspacemat}{\bds{B}}
\newcommand{\nullspacematArg}[1]{\nullspacemat_{#1}}
\newcommand{\nullspacemati}{\nullspacematArg{i}}

\newcommand{\redNullspacemat}{\hat{\bds{B}}}
\newcommand{\redNullspacematArg}[1]{\redNullspacemat_{#1}}
\newcommand{\redNullspacemati}{\redNullspacematArg{i}}

\newcommand{\identityi}{\bds{E}_i}
\newcommand{\uncoupledMiniNo}{g_i}
\newcommand{\uncoupledMini}[1]{\uncoupledMiniNo(#1)}
\newcommand{\lagrange}{\bds{\lambda}}
\newcommand{\lagrangian}{L}
\newcommand{\zero}{\bds{0}}
\newcommand{\argmin}[1]{\underset{#1}{\text{arg min}}}
\newcommand{\range}[1]{\mathrm{range}(#1)}
%\newcommand{\diag}[1]{\text{diag}(#1)}
\newcommand{\subdomainPorts}[1]{P(#1)}
\newcommand{\portsSubdomains}[1]{Q(#1)}
\newcommand{\portsSubdomainsTwo}[2]{Q(#1,#2)}
\newcommand{\nports}{{n_p}}
\newcommand{\nportsSub}[1]{{\nports(#1)}}
\newcommand{\ndofPorts}[1]{n^p}
\newcommand{\ndofPortsArg}[1]{n_{#1}^p}
\newcommand{\ndofPortsj}{\ndofPortsArg{j}}
\newcommand{\projectionStatePort}[2]{\projection^{#1}_{#2}}
\newcommand{\projectionStatePortAll}[1]{\projection^{#1}}
\newcommand{\nconstraintsPort}[1]{n^c_{#1}}
%\newcommand{\card}[1]{\text{card}(#1)}
\newcommand{\card}[1]{|#1|}
\newcommand{\RRstar}[1]{\mathbb{R}_\star^{#1}}
\newcommand{\directSumLimits}[1]{\underset{#1}{\mathlarger{\mathlarger{\oplus}}}}
\newcommand{\sampleSpaceGenCoord}{\mathcal D_{\redsolapproxST}}
\newcommand{\assLipschitz}{$(\bf{A}_1)$}
%\newcommand{\assInvLipschitz}{$(\bf{A}_3)$}
\newcommand{\assBounded}{$(\bf{A}_3)$}
\newcommand{\asssmallDt}{$(\bf{A}_2)$}
\newcommand{\asssmallDtNonlin}{$(\bf{A}_4)$}
\newcommand{\sigmamax}[1]{\sigma_\mathrm{max}(#1)}
\newcommand{\sigmamin}[1]{\sigma_\mathrm{min}(#1)}
\newcommand{\normEquiv}{P}
\newcommand{\lebesgue}{\Lambda}


%\newtheorem{theorem}{Theorem}
%\newtheorem{corollary}{Corollary}
%\newtheorem{lemma}{Lemma}

%\newenvironment{proof}{\begin{trivlist}
%\item {\emph {Proof}:\:}}
%{$\square$\end{trivlist}}

%\newenvironment{definition}[1]{\begin{trivlist}
%\item {{\emph {#1}}:\:}}
%{$\square$\end{trivlist}}
%
%\newcounter{lemctr}
%\setcounter{lemctr}{0}
%\newenvironment{lemma}{\refstepcounter{lemctr}\begin{trivlist}
%\item {\sc {Lemma~\arabic{lemctr}}.\:}}
%{$\blacksquare$\end{trivlist}}
%
%\newcounter{pfctr}
%\setcounter{pfctr}{0}
%\newenvironment{longproof}{\refstepcounter{pfctr}\begin{trivlist}
%\item {\sc {Proof \arabic{pfctr}}:\:}}
%{$\blacksquare$\end{trivlist}}
%
\newcounter{remctr}
\setcounter{remctr}{0}
%\newenvironment{remark}{\refstepcounter{remctr}\begin{trivlist}
%\item {\emph {Remark}.\:}}
%{$\blacksquare$\end{trivlist}}

%\newcounter{examplectr}
%\setcounter{examplectr}{0}
%\newenvironment{example}{\refstepcounter{examplectr}\begin{trivlist}
%\item {\emph {Example}.\:}}
%{$\blacksquare$\end{trivlist}}

\newcounter{propctr}
\setcounter{propctr}{0}
\newenvironment{property}{\refstepcounter{propctr}\begin{trivlist}
\item {\sc {Property \arabic{propctr}}.\:}}
{$\blacksquare$\end{trivlist}}

\newcounter{proposctr}
\setcounter{proposctr}{0}
\newenvironment{propos}{\refstepcounter{proposctr}\begin{trivlist}
\item {\sc {Proposition \arabic{proposctr}}.\:}}
{$\blacksquare $\end{trivlist}}
\newenvironment{proofofthing}[2]{\begin{trivlist}
\item {\sc {Proof of #1 \ref{#2}}.\:}}
{$\blacksquare $\end{trivlist}}


\newcommand{\RR}[1]{\ensuremath{\mathbb{R}^{ #1 }}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\RRplus}[1]{\ensuremath{\mathbb{R}_+^{ #1 }}}
\newcommand{\natNo}{\NN}
\newcommand{\nat}[1]{\natNo\,\pa{#1}}
\newcommand{\natZero}[1]{\{0,\ldots,#1\}}
\newcommand{\innat}[1]{\in\nat{#1}}
\newcommand{\innatSeq}[1]{=1,\ldots,#1}
\newcommand{\innatZero}[1]{\in\natZero{#1}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\Image}[1]{\mathrm{Im}\left(#1\right)}
\newcommand{\Span}[1]{\mathrm{span}\left\{#1\right\}}
%\newcommand{\Range}[1]{\mathrm{Ran}\left(#1\right)}
\newcommand{\vecmat}[2]{\bmat{#1^1 & \cdots& #1^{#2}}}
\newcommand{\entryvec}[3]{\left[#1_{#3_1} \ \cdots\ #1_{#3_{#2}}\right]^T}
\newcommand{\identity}[1]{\boldsymbol I_{#1}}
\newcommand{\nstepExtraction}{P_n}
\newcommand{\lipschitz}{\kappa}
\newcommand{\lipschitzst}{\bar{\lipschitz}}

\newcommand{\pexit}{P_\text{exit}}
\newcommand{\specificheat}{\gamma}
\newcommand{\energypermass}{\epsilon}
\newcommand{\densitySymb}{\rho}
\newcommand{\velocitySymb}{u}
\newcommand{\energydensity}{e}
\newcommand{\pressureSymb}{p}
\newcommand{\specificgasconstant}{R}
\newcommand{\speedofsoundSymb}{c}
\newcommand{\machSymb}{M}
\newcommand{\temperatureSymb}{T}
\newcommand{\resSymb}{r}
\newcommand{\resRedSymb}{{\mathsf r}}
\newcommand{\fluxSymb}{f}
\newcommand{\paramSymb}{\mu}
\newcommand{\solSymb}{u}
\newcommand{\tensor}{\pmb{\mathscr{X}}}

\newcommand{\tensorSub}[1]{\tensor_{\!\!#1}}
\newcommand{\tensorSubSubWindowArg}[3]{\tensor_{\!\!#1}^{#2,#3}}

\newcommand{\tensorSubP}[1]{\bm{\mathscr{P}}_{\!\!#1}}
\newcommand{\tensorSubRes}[1]{\bm{\mathscr{R}}_{\!\!#1}}
\newcommand{\tensorUnfold}[1]{\snapshots_{(#1)}}

\newcommand{\numGaussNewtonIterationsArg}[2]{n_{\text{GN}}^{#1,#2}}

\newcommand{\residTensorSubWindowArg}[2]{\bm{\mathscr{R}}^{#1,#2} }

\newcommand{\stateTensorSubWindowArg}[2]{\tensor_{\!\!\bm{u}}^{#1,#2} }
\newcommand{\stateTensorUnfoldSubWindowArg}[3]{\snapshots^{\!\!\!\!#2,#3}_{(#1)}}

\newcommand{\stateTensorSTHOSVDSubWindowArg}[3]{\tensor_{\bm{u}}^{#1,#2}(#3) }
\newcommand{\stateTensorSTHOSVDUnfoldSubWindowArg}[4]{\snapshots_{(#1)}^{\!\!\!\!#2,#3}(#4)}
\newcommand{\stateTensorTSTHOSVDSubWindowArg}[3]{\tensor_{\!\!\bm{u}}^{#1,#2}(#3) }
\newcommand{\stateTensorTSTHOSVDUnfoldSubWindowArg}[4]{\snapshots_{(#1)}^{\!\!\!\!#2,#3}(#4)}

\newcommand{\tensorReduceNo}{\mathcal X}
\newcommand{\tensorReduce}[1]{\tensorReduceNo(#1)}
\newcommand{\tensorresReduce}[1]{\tensorresReduceNo(#1)}
\newcommand{\tensorReduceUnfold}[2]{\snapshots(#1)_{(#2)}}
\newcommand{\tensorres}{\mathcal R}
\newcommand{\tensorresUnfold}[1]{\boldsymbol{R}_{(#1)}}
\newcommand{\tensorresReduceNo}{\mathcal R}
\newcommand{\tensorresReduceUnfold}[2]{\boldsymbol{R}(#1)_{(#2)}}
\newcommand{\dummyBasisDiscrete}{\bm{\mathsl{v}}}
\newcommand{\dummyTestDiscrete}{\bm{\mathsl{w}}}
\newcommand{\dummyFullDiscrete}{\bm{\mathsl{y}}}
\newcommand{\dummyFullDiscreteArg}[1]{\bm{\mathsl{y}}^{#1}}
\newcommand{\dummyWindowDiscreteArg}[2]{\bm{\mathsl{y}}^{#1,#2}}

\newcommand{\dummyFullDiscreteScalarArg}[1]{\mathsl{y}^{#1}}
\newcommand{\fluxFullDiscreteArg}[1]{\bm{\mathsl{f}}^{#1}}
\newcommand{\tbasismat}{\bm{\mathit{\Psi}}}
\newcommand{\tbasismatSubWindowArg}[2]{\tbasismat^{#1,#2}}
\newcommand{\NA}{---}
\newcommand{\solTimeContinuous}{\bm{u}}
\newcommand{\resTimeContinuous}{\bm{r}}
\newcommand{\solFullDiscrete}{\bm{\mathsl{u}}}
\newcommand{\dumFullDiscrete}{\bm{\mathsl{v}}}
\newcommand{\solFullDiscreteArg}[1]{\bm{\mathsl{u}}^{#1}}
\newcommand{\solFullDiscreteTransposeArg}[1]{\bm{\mathsl{u}}^{{#1}^{\T}}}
\newcommand{\dumFullDiscreteArg}[1]{\dumFullDiscrete^{#1}}
\newcommand{\dumFullDiscreteTransposeArg}[1]{\dumFullDiscrete^{{#1}^{\T}}}
\newcommand{\solFullDiscreteApproxArg}[1]{\widetilde{\bm{\mathsl{u}}}^{#1}}
\newcommand{\resFullDiscreteApproxArg}[1]{\widetilde{\bm{\mathsl{r}}}^{#1}}
\newcommand{\solFullDiscreteApproxHarpoonArg}[1]{\overrightharpoon{\bm{\mathsl{u}}}^{#1}}

\newcommand{\solFullDiscreteReduced}{\goodhat{\bm{\mathsl{u}}}}
\newcommand{\dummyFullDiscreteReduced}{\goodhat{\bm{\mathsl{y}}}}
\newcommand{\trialFullDiscrete}{\bm{\mathsl{v}}}
\newcommand{\trialFullDiscreteArg}[1]{\trialFullDiscrete^{#1}}
\newcommand{\dummyFullDiscreteReducedArg}[1]{\dummyFullDiscreteReduced^{#1}}
\newcommand{\timeContinuousSpace}{\mathpzc{T}}
\newcommand{\timeContinuousSpaceWin}{\timeContinuousSpace^k}
\newcommand{\timeContinuousSpaceWinDD}{\timeContinuousSpace^m}
\newcommand{\timeContinuousSpaceWinNeg}{\timeContinuousSpace^{k-1}}

\newcommand{\solFullDiscreteReducedArg}[1]{\goodhat{\bm{\mathsl{u}}}^{#1}}
\newcommand{\resFullDiscrete}{\bm{\mathsl{r}}}
\newcommand{\resFullSTDiscrete}{\overrightarrow{\bm{\mathsl{r}}}}
\newcommand{\resFullWSTDiscreteArg}[1]{\resFullSTDiscrete^{#1}}

\newcommand{\resFullDiscreteArg}[1]{\bm{\mathsl{r}}^{#1}}
\newcommand{\resWindowDiscreteArg}[2]{\bm{\mathsl{r}}^{#1,#2}}

\newcommand{\solFullDiscreteOnlyParam}{\solFullDiscrete(\param)}
\newcommand{\solapproxFullDiscrete}{\tilde\mathbf{x}}
\newcommand{\solapproxFullDiscreteOnlyParam}{\tilde{\mathbf{x}}(\param)}
\newcommand{\solapproxSTFullDiscrete}{\tilde\mathbf{x}_\text{ST}}
\newcommand{\solapproxSTFullDiscreteOnlyParam}{\tilde{\mathbf{x}}_\text{ST}(\param)}
\newcommand{\unknownSymb}{w}
\newcommand{\spaceSymb}{s}
\newcommand{\timeSymb}{t}
\newcommand{\timestepit}{n}
\newcommand{\singvalmatSymb}{\Sigma}
\newcommand{\leftsingmatSymb}{U}
\newcommand{\rightsingmatSymb}{V}
\newcommand{\leftsingvecSymb}{u}
\newcommand{\rightsingvecSymb}{v}
\newcommand{\rearrangedrightsingvecspaceSymb}{K}
\newcommand{\weightmatSymb}{A}
\newcommand{\weightvecSymb}{a}
\newcommand{\basismatspaceSymb}{\Phi}
\newcommand{\basisvecspaceSymb}{\phi}
\newcommand{\basismattimeSymb}{\Psi}
\newcommand{\basisvectimeSymb}{\psi}
\newcommand{\basisvectimeFuncSymb}{\uppsi}
\newcommand{\basismatstSymb}{\Upsilon}
\newcommand{\basisvecstSymb}{\upsilon}
\newcommand{\operatorerroboundSymb}{\Xi}
\newcommand{\samplematSymb}{Z}
\newcommand{\samplevecSymb}{z}
\newcommand{\dummySymb}{y}
\newcommand{\snapshotSymb}{{X_u}}
\newcommand{\snapshotApproxSymb}{\bm{X}_{\widetilde{\bm{u}}}}
\newcommand{\snapshotReducedSymb}{\bm{X}_{\hat{\bm{u}}}}
\newcommand{\snapshotResSymb}{X_r}
\newcommand{\snapshotmatspaceSymb}{A}
\newcommand{\snapshotmattimeSymb}{B}
\newcommand{\stabilityconstantSymb}{h}

\newcommand{\nparam}{n_\mu}
\newcommand{\ntrain}{n_\text{train}}
\newcommand{\nparamROM}{n_{\hat\paramSymb}}
\newcommand{\nrestrain}{n_\text{res}}
\newcommand{\nressample}{n_{\samplevecSymb}}
\newcommand{\nressamplest}{\bar n_{\samplevecSymb}}
\newcommand{\nressamplestSmall}{\bar n_{\samplevecSymb}'}
\newcommand{\nrestimeind}{\bar n_{\timeSymb}}
\newcommand{\nresspaceind}{\bar n_{\spaceSymb}}
\newcommand{\nbasisres}{n_\resSymb}
\newcommand{\nbasisresst}{\bar n_\resSymb}
%\newcommand{\nbasisspace}{n_\basisvecspaceSymb}
%\newcommand{\nbasistime}{n_\basisvectimeSymb}
\newcommand{\nbasisspace}{{n_\spaceSymb}}
\newcommand{\nbasisspaceres}{{n_{\resSymb,\spaceSymb}}}
\newcommand{\nbasistime}{n_\timeSymb}
\newcommand{\nbasistimeres}{n_{\resSymb,\timeSymb}}
\newcommand{\nbasisst}{{n_{\spaceSymb\timeSymb}}}
\newcommand{\nbasisstTensor}{\sum_{i=1}^{\nbasisspace}\nbasistime^i}
\newcommand{\nspacedof}{N_\spaceSymb}
\newcommand{\ntimedof}{{N_\timeSymb}}
\newcommand{\ntimedofWin}{{N_{\timeSymb}^k}}
\newcommand{\numStepsInWindow}{N_{\timeSymb}^k}
\newcommand{\numStepsInWindowArg}[1]{N_{\timeSymb}^{#1}}
\newcommand{\ntimedofSubWin}{{N_{\timeSymb}^{k,m}}}
\newcommand{\nTimestepsFine}{\ntimedof}
%\newcommand{\nspacedof}{N}
%\newcommand{\ntimedof}{M}

\newcommand{\paramDomain}{\mathcal D}
%\newcommand{\paramDomainTrain}{\overline\paramDomain}
\newcommand{\paramDomainTrain}{\paramDomain_\text{train}}
\newcommand{\paramDomainTrainResid}{\paramDomain_\text{train,r}}

\newcommand{\paramDomainTrainres}{\paramDomain_\text{res}}
\newcommand{\ones}{\onebold}
\newcommand{\onesFunc}{\mathcal{O}}
\newcommand{\totaltime}{T}
\newcommand{\VS}{\mathrm{S}}
\newcommand{\trialSSubspaceColumn}{\mathpzc{V}_{\VS_0}}
\newcommand{\trialSSubspace}{\mathpzc{V}_\VS}
\newcommand{\testSSubspaceColumn}{\mathpzc{W}_{\VS_0}}
\newcommand{\testSSubspace}{\mathpzc{W}_\VS}
\newcommand{\trialSTSubspace}{{\mathpzc{V}_{\vST}}}
\newcommand{\trialSTSubspaceColumn}{\mathpzc{V}_{\mathrm{ST}_0}}
\newcommand{\trialSTSubspaceWin}{\mathpzc{V}_{\vST}^k}
\newcommand{\trialSTSubspaceWinNeg}{\mathpzc{V}_{\vST}^{k-1}}
\newcommand{\trialSTSubspaceColumnWin}{\mathpzc{V}_{\vST_0}^k}
\newcommand{\trialSTSubspaceWinDD}{\mathpzc{V}_{\vST}^{k,m}}
% \newcommand{\trialSTSubspaceSubWinTensor}{\overrightharpoon{\mathpzc{V}}_{ST}^{k,m}}
\newcommand{\trialSTSubspaceWinDDV}[1]{\mathpzc{V}_{\vST}^{k,#1}}
\newcommand{\trialSTSubspaceColumnWinDD}{\mathpzc{V}_{\vST_0}^{k,m}}
\newcommand{\testSTSubspace}{\mathpzc{W}_{\ST}}
\newcommand{\testSTSubspaceColumn}{\mathpzc{W}_{\ST_0}}
\newcommand{\temporalSubspaceFunc}{\fontDiscreteFunc T}
\newcommand{\temporalSubspace}{\fontDiscrete T}
\newcommand{\spatiotemporalSubspaceFunc}{\fontDiscreteFunc{ST}}
\newcommand{\spatiotemporalSubspace}{\fontDiscrete{ST}}
%\newcommand{\spacesampleset}{\spatialSubspace_{r}}
%\newcommand{\timesampleset}{\temporalSubspace_{r}}
\newcommand{\spacesampleset}{\mathfrak{s}}
\newcommand{\timesampleset}{\mathfrak{t}}
\newcommand{\PG}{\text{PG}}
\newcommand{\Tbe}{\boldsymbol A_\text{BE}}
\newcommand{\Alm}{\boldsymbol A_\text{LM}}
\newcommand{\Blm}{\boldsymbol B_\text{LM}}
\newcommand{\objective}{\zeta}
\newcommand{\operatorerrorboundSymb}{\Lambda}

\newcommand{\stabilityconstantBE}{\bar{\stabilityconstantSymb}_\text{be}}
\newcommand{\stabilityconstantLM}{\bar{\stabilityconstantSymb}_\text{lm}}
\newcommand{\tn}{\timeSymb^n}
\newcommand{\tnm}{\timeSymb^{n-1}}
\newcommand{\resSymbst}{\bar{\resSymb}}
\newcommand{\resRedSymbst}{\bar{\resRedSymb}}
\newcommand{\res}{\boldsymbol \resSymb}
\newcommand{\resk}{\boldsymbol \resSymb_k}
\newcommand{\reskn}{\boldsymbol \resSymb_{k(n)}}
\newcommand{\resArg}[1]{\boldsymbol \resSymb^{#1}}
\newcommand{\resArgEntry}[2]{\resSymb_{#1}^{#2}}
%\newcommand{\resRedArg}[1]{\boldsymbol \resRedSymb^{#1}}
\newcommand{\resRed}{\boldsymbol \resRedSymb}
\newcommand{\resRedApprox}{\tilde{\boldsymbol \resRedSymb}}
\newcommand{\resRedArg}[1]{\resRed(t^{#1})}
\newcommand{\resn}{\resArg{n}}
\newcommand{\resst}{\boldsymbol \resSymbst}
\newcommand{\resstApprox}{\tilde {\res}}
\newcommand{\resRedst}{\boldsymbol \resRedSymbst}
\newcommand{\resRedstapprox}{\bar{\tilde{\boldsymbol \resRedSymb}}}
\newcommand{\param}{\boldsymbol \paramSymb}
\newcommand{\paramTrain}[1]{\param^{#1}_\text{train}}
\newcommand{\paramTrainres}[1]{\param^{#1}_\text{res}}
\newcommand{\paramDummy}{\boldsymbol \mu}
\newcommand{\dt}{\Delta \timeSymb}
\newcommand{\dtArg}[1]{\reviewerA{\dt^{#1}}}
\newcommand{\sol}{\boldsymbol \solSymb}
\newcommand{\solw}{\boldsymbol u}
% \newcommand{\solTimeContinuous}{\sol^\star}
\newcommand{\solst}{\bar{\sol}}
\newcommand{\solSymbst}{\bar{\solSymb}}
\newcommand{\flux}{\boldsymbol \fluxSymb}
\newcommand{\rhs}{\bar{\boldsymbol b}}
\newcommand{\rhsFunc}{\boldsymbol b}
\newcommand{\rhsFuncArg}[1]{\rhsFunc(t^{#1})}
\newcommand{\fluxst}{\bar{\flux}}
\newcommand{\solfom}{\sol_\star}
\newcommand{\solpgst}{\solst_{PG}}
\newcommand{\solfomst}{\solst_\star}
\newcommand{\solDummyScalar}{ u}
\newcommand{\solDummyScalarArg}[1]{\solDummyScalar^{#1}}
\newcommand{\solDummyScalarFuncArg}[1]{\solDummyScalar(t^{#1})}
\newcommand{\solDummy}{\boldsymbol u}
\newcommand{\solDummyst}{\bar\solDummy}
\newcommand{\solDummyArg}[1]{\solDummy^{#1}}
\newcommand{\solDummyFuncArg}[1]{\solDummy(t^{#1})}
\newcommand{\solDummyFuncArgDummy}[1]{\solDummy(\timeDummy^{#1})}
\newcommand{\solDummyOptFuncArg}[1]{\solDummyOpt(t^{#1})}
\newcommand{\solRedDummyScalar}{ \hat w}
\newcommand{\solRedDummyScalarArg}[1]{\solRedDummyScalar_{#1}}
\newcommand{\solRedDummy}{\hat {\boldsymbol w}}
\newcommand{\solDummyOpt}{{\boldsymbol \optDummy}}
\newcommand{\solRedDummyOpt}{\hat {\boldsymbol \optDummy}}
\newcommand{\timeArg}[1]{t^{#1}}
\newcommand{\timeDummy}{\tau}
\newcommand{\timeDomain}{[0,\totaltime]}
%\newcommand{\timestepset}{\mathfrak t}
\newcommand{\timestepset}{\{\timeArg{n}\}_{n=0}^{\ntimedof}}
\newcommand{\solFunc}{\sol}
\newcommand{\solinfty}{\sol_\infty}
\newcommand{\soltwo}{\sol_2}
\newcommand{\solFuncArg}[1]{\solFunc(t^{#1};\param)}
\newcommand{\solFuncOnlyParam}{\solFunc(\cdot;\param)}
\newcommand{\solFuncOnlyParamTrain}[1]{\solFunc(\cdot;\paramTrain{#1})}
\newcommand{\solFuncOnlyParamProject}{\hat\solFunc(\param)}
\newcommand{\solFuncOnlyParamProjectArg}[2]{\hat\solSymb_{#1#2}(\param)}
\newcommand{\solFuncn}{\solFuncArg{n}}
\newcommand{\solFuncnm}{\solFuncArg{n-1}}
%\newcommand{\solArg}[1]{\sol^{#1}(\param)}
\newcommand{\solArg}[1]{\sol(t^{#1};\param)}
\newcommand{\soln}{\solArg{n}}
\newcommand{\solnm}{\solArg{n-1}}
\newcommand{\spacetimesubspaceFunc}{\mathcal{S}\mathcal{T}}
\newcommand{\spacetimesubspace}{\fontDiscrete{ST}}
\newcommand{\spacetimesubspacesmall}{\mathcal{ST}'}

\newcommand{\solapproxFunc}{\solapprox}
\newcommand{\solapproxFuncArg}[1]{\solapproxFunc(t^{#1};\param)}
\newcommand{\solapproxFuncArgs}[2]{\solapproxFunc_\text{#1}(t^{#2};\param)}
\newcommand{\solapproxFuncOnlyParam}{\solapproxFunc(\cdot;\param)}
\newcommand{\solapproxFuncn}{\solapproxFuncArg{n}}
\newcommand{\solapproxFuncnm}{\solapproxFuncArg{n-1}}

\newcommand{\redsolapproxFunc}{\redsolapprox}
\newcommand{\redsolapproxFuncArg}[1]{\redsolapproxFunc(t^{#1};\param)}
\newcommand{\redsolapproxFuncArgGen}[1]{\redsolapproxFunc(#1;\param)}
\newcommand{\redsolapproxFuncOnlyParam}{\redsolapproxFunc(\cdot;\param)}
\newcommand{\redsolapproxFuncn}{\redsolapproxFuncArg{n}}
\newcommand{\redsolapproxFuncnm}{\redsolapproxFuncArg{n-1}}

\newcommand{\redsolapproxEntryFunc}{\hat{\boldsymbol{u}}}
\newcommand{\redsolapproxEntryFuncArg}[2]{\redsolapproxEntryFunc_{#1}(t^{#2};\param)}
\newcommand{\redsolapproxEntryFuncArgGen}[2]{\redsolapproxEntryFunc_{#1}(#2;\param)}
\newcommand{\redsolapproxEntryFuncOnlyParam}[1]{\redsolapproxEntryFunc_{#1}(\cdot;\param)}
\newcommand{\redsolapproxEntryFuncn}{\redsolapproxEntryFuncArg{n}}
\newcommand{\redsolapproxEntryFuncnm}{\redsolapproxEntryFuncArg{n-1}}




\newcommand{\lineSearchParam}{\alpha}
\newcommand{\lineSearchParamArg}[1]{\lineSearchParam^{(#1)}}
\newcommand{\testbasis}{\boldsymbol \Xi}
\newcommand{\testbasisArg}[2]{\boldsymbol \xi_{ij}}


%\newcommand{\solapproxArg}[1]{\solapprox^{#1}(\param)}
\newcommand{\solapproxArg}[1]{\solapprox(t^{#1};\param)}
\newcommand{\solapproxArgs}[2]{\solapprox_\text{#1}(t^{#2};\param)}
\newcommand{\solapproxn}{\solapproxArg{n}}
\newcommand{\solapproxnm}{\solapproxArg{n-1}}

\newcommand{\redsolapproxArg}[1]{\redsolapprox(t^{#1};\param)}
\newcommand{\redsolapproxn}{\redsolapproxArg{n}}
\newcommand{\redsolapproxnm}{\redsolapproxArg{n-1}}

\newcommand{\paramTrainInitial}{\paramDomain_\text{initial}}
\newcommand{\paramTrainInitialArg}[1]{\param_\text{initial}^{#1}}
\newcommand{\nparamTrainInitial}{{n_{\paramSymb,\text{initial}}}}

%\newcommand{\pa}[1]{(#1)}
\newcommand{\solSTscalar}{u}
\newcommand{\solST}{\boldsymbol{\solSTscalar}}
\newcommand{\solapproxSTFunc}{\tilde\solST}
\newcommand{\solapproxST}{\tilde\solST}
\newcommand{\solapproxSTFuncArg}[1]{\solapproxSTFunc(t^{#1};\param)}
\newcommand{\solapproxSTFuncArgs}[2]{\solapproxSTFunc_\text{#1}(t^{#2};\param)}
\newcommand{\solapproxSTFuncOnlyParam}{\solapproxSTFunc(\cdot;\param)}
\newcommand{\solapproxSTFuncn}{\solapproxSTFuncArg{n}}
\newcommand{\solapproxSTFuncnm}{\solapproxSTFuncArg{n-1}}
\newcommand{\solapproxSTArg}[1]{\solapproxSTFunc^{#1}(\param)}
\newcommand{\solapproxSTn}{\solapproxSTArg{n}}
\newcommand{\solapproxSTnm}{\solapproxSTArg{n-1}}

\newcommand{\redsolapproxST}{\hat\solST}
\newcommand{\redsolapproxSTVecArg}[1]{\redsolapproxST_{#1}(\param)}
\newcommand{\redsolapproxSTArg}[1]{\hat\solSTscalar_{#1}(\param)}
\newcommand{\redsolapproxSTArgNone}[1]{\hat\solSTscalar_{#1}}
\newcommand{\redsolapproxSTIt}[1]{\hat\solST^{(#1)}}
\newcommand{\deltaredsolapproxSTIt}[1]{\delta\hat\solST^{({#1})}}
\newcommand{\redsolapproxTrainNo}{\hat\solST_\text{res}}
\newcommand{\redsolapproxTrainArg}[1]{\redsolapproxTrainNo^{#1}}
\newcommand{\redsolapproxFOMTrainNo}{\hat\solST_\text{FOM}}
\newcommand{\redsolapproxFOMTrainArg}[1]{\redsolapproxFOMTrainNo(\paramTrain{#1})}
\newcommand{\redsolapproxFOMTrain}{\redsolapproxFOMTrainNo(\param)}
\newcommand{\stbasismat}{\bm{\mathit{\Pi}}}
\newcommand{\stbasismatResid}{\bm{\mathit{\Pi}}_{R}}
\newcommand{\stbasismatResidArg}[1]{\bm{\mathit{\Pi}}_{r}^{#1}}
\newcommand{\residualBasisDimWSTArg}[1]{n_{st,r}^{#1}}
\newcommand{\wstbasismatArg}[1]{\bm{\mathit{\Pi}}^{#1}}

\newcommand{\residualReducedWindowArg}[1]{\widehat{\bm{ \mathsl{r}}}_g^{#1}}
\newcommand{\stbasismatSubWindowArg}[2]{\stbasismat^{#1,#2}}
\newcommand{\stbasismatEndSubWindowArg}[2]{\overline{\stbasismat}^{#1,#2}}


\newcommand{\stbasismatWindowArg}[1]{\stbasismat^{#1}}
\newcommand{\stbasismatWinDD}{\bm{\mathit{\Pi}}_k^{m}}
\newcommand{\sbasismat}{\!\bm{\mathit{\Phi}}}
\newcommand{\sbasismatSubWindowArg}[2]{\!\bm{\mathit{\Phi}}^{#1,#2}}

\newcommand{\stbasisvec}[1]{\boldsymbol \pi_{#1}}
\newcommand{\stbasisvecR}[1]{\boldsymbol \pi_{r, #1}}
\newcommand{\stbasisvecFunc}[1]{\boldsymbol \uppi_{#1}}
\newcommand{\mseError}{\text{relative error}}

\newcommand{\stestmat}{\!\bm{\mathit{\Upsilon}}}

\newcommand{\romdim}{n_s}
\newcommand{\romdimST}{n_{st}}
\newcommand{\romdimWSTArg}[1]{\romdimST^{#1}}
\newcommand{\romdimWSTSubWindowArg}[2]{\romdimST^{#1,#2}}


\newcommand{\solnfom}{\soln_\star}
\newcommand{\solnpg}{\sol_{PG}^n}
\newcommand{\solnmfom}{\sol_\star^{n-1}}
\newcommand{\solapprox}{\tilde\sol}
\newcommand{\redsolapprox}{\hat\sol}
\newcommand{\solapproxPG}{\solapprox_\PG}
\newcommand{\redsol}{\hat\sol}
\newcommand{\redsoln}{\redsol^n}
\newcommand{\redsolst}{\redsol}
\newcommand{\redsolstSol}{\redsol_\star}
\newcommand{\redsolstij}[2]{\hat\solSymb_{#1#2}}
\newcommand{\soli}[1]{\sol^{#1}}
\newcommand{\solEntry}[1]{\solSymb_{#1}}
\newcommand{\resEntryi}[1]{\resSymb_{#1}}
\newcommand{\resRedEntryi}[1]{\mathsf\resSymb_{#1}}
\newcommand{\unknown}{\boldsymbol{\unknownSymb}}
\newcommand{\unknowni}[1]{\unknown_{#1}}
\newcommand{\dummy}{\boldsymbol {\dummySymb}}
\newcommand{\reddummy}{\hat{\dummy}}
\newcommand{\reddummyij}[2]{\hat{\dummySymb}_{#1#2}}
\newcommand{\redres}{\hat{\res}}
\newcommand{\solinit}{\sol^0}
\newcommand{\solinitEntry}[1]{\solSymb_{#1}^0}
\newcommand{\solinitst}{\bar{\sol}^0}
\newcommand{\solref}{\solFullDiscrete_{\mathrm{ref}}}
\newcommand{\solrefST}{\overrightharpoon{\solFullDiscrete}_{\mathrm{ref}_{\ST}}}
%\newcommand{\solref}{\solinit(\param)}
\newcommand{\solrefst}{\bar{\sol}_{\text{ref}}}
\newcommand{\singvalmat}{\boldsymbol \singvalmatSymb}
\newcommand{\singvalmatspace}{\singvalmat_\spaceSymb}
\newcommand{\singvalmatspaceSubWindowArg}[2]{\singvalmat_\spaceSymb^{#1,#2}}

\newcommand{\singvalmatspaceres}{\singvalmat_{\resSymb,\spaceSymb}}
\newcommand{\singvalmattime}{\singvalmat_\timeSymb}
\newcommand{\singvalmattimeres}{\singvalmat_{\resSymb,\timeSymb}}
\newcommand{\leftsingvec}{\boldsymbol{\leftsingvecSymb}}
\newcommand{\rightsingvec}{\boldsymbol{\rightsingvecSymb}}
\newcommand{\leftsingvecspace}{\leftsingvec_\spaceSymb}
\newcommand{\leftsingvecspaceres}{\leftsingvec_{\resSymb,\spaceSymb}}
\newcommand{\leftsingvectime}{\leftsingvec_\timeSymb}
\newcommand{\leftsingvectimeres}{\leftsingvec_{\resSymb,\timeSymb}}
\newcommand{\leftsingvectimeArg}[1]{\leftsingvectime^{#1}}
\newcommand{\leftsingvectimeresArg}[1]{\leftsingvectimeres^{#1}}
\newcommand{\rightsingvecspace}{\rightsingvec_\spaceSymb}
\newcommand{\rightsingvectime}{\rightsingvec_\timeSymb}
\newcommand{\leftsingvecspacei}[1]{\leftsingvecspace^{#1}}
\newcommand{\leftsingvecspaceresi}[1]{\leftsingvecspaceres^{#1}}
\newcommand{\leftsingvectimei}[1]{\leftsingvectime^{#1}}
\newcommand{\leftsingvectimeij}[2]{\leftsingvectime^{#1,#2}}
\newcommand{\rightsingvecspacei}[1]{\rightsingvecspace^{#1}}
\newcommand{\rightsingvecspaceij}[2]{\rightsingvec_{\spaceSymb,#2}^{#1}}
\newcommand{\rightsingvectimei}[1]{\rightsingvectime^{#1}}
\newcommand{\rightsingvecspaceSymbij}[2]{\rightsingvecSymb_{\spaceSymb,#1}^{#2}}
\newcommand{\leftsingmat}{\boldsymbol{\leftsingmatSymb}}

\newcommand{\rightsingmat}{\boldsymbol{\rightsingmatSymb}}
\newcommand{\leftsingmatspace}{\leftsingmat_\spaceSymb}
\newcommand{\leftsingmatspaceSubWindowArg}[2]{\leftsingmat_\spaceSymb^{#1,#2}}
\newcommand{\leftsingmatspaceres}{\leftsingmat_{\resSymb,\spaceSymb}}
\newcommand{\leftsingmattime}{\leftsingmat_\timeSymb}
\newcommand{\leftsingmattimei}[1]{\leftsingmattime^{#1}}
\newcommand{\leftsingmattimeres}{\leftsingmat_{\resSymb,\timeSymb}}
\newcommand{\leftsingmattimeresi}[1]{\leftsingmattimeres^{#1}}
\newcommand{\rightsingmatspace}{\rightsingmat_\spaceSymb}
\newcommand{\rightsingmatspaceSubWindowArg}[2]{\rightsingmat_\spaceSymb^{#1,#2}}

\newcommand{\rightsingmatspaceres}{\rightsingmat_{\resSymb,\spaceSymb}}
\newcommand{\rightsingmattime}{\rightsingmat_\timeSymb}
\newcommand{\nnzNo}{\mathrm{nnz}}
\newcommand{\nnz}[1]{\nnzNo(#1)}
\newcommand{\rightsingmattimeres}{\rightsingmat_{\resSymb,\timeSymb}}
\newcommand{\rightsingmattimei}[1]{\rightsingmattime^{#1}}
\newcommand{\rearrangedrightsingvecspace}{\boldsymbol \rearrangedrightsingvecspaceSymb}
\newcommand{\rearrangedrightsingvecspacei}[1]{\rearrangedrightsingvecspace^{#1}}
\newcommand{\basismattime}{\boldsymbol{\basismattimeSymb}}
\newcommand{\basismattimei}[1]{\basismattime^{#1}}
\newcommand{\basisvectime}{\boldsymbol{\basisvectimeSymb}}
\newcommand{\basisvectimei}[1]{\basisvectime_{#1}}
\newcommand{\basisvectimeij}[2]{\basisvectime^{#1}_{#2}}
\newcommand{\basisvectimeijk}[3]{{\basisvectimeSymb}^{#1}_{#2#3}}
\newcommand{\basisvectimeresi}[1]{\basisvectime_{r,#1}}
\newcommand{\basisvectimeresij}[2]{\basisvectime^{#1}_{r,#2}}
\newcommand{\basisvectimeresijk}[3]{{\basisvectimeSymb}^{#1}_{r,#2#3}}
\newcommand{\basisvectimeFunc}{\boldsymbol{\basisvectimeFuncSymb}}
\newcommand{\basisvectimeFuncij}[2]{\basisvectimeFunc_{#2}^{#1}}
\newcommand{\basisvectimeresFuncij}[2]{\basisvectimeFunc_{r,#2}^{#1}}
\newcommand{\basisvectimeFunci}[1]{\basisvectimeFunc_{#1}}
\newcommand{\basisvectimeresFunci}[1]{\basisvectimeFunc_{r,#1}}
\newcommand{\basisvectimeFuncVeci}[1]{\basisvectimeFunc^{#1}}
\newcommand{\basisvectimeFuncijk}[3]{{\basisvectimeFuncSymb}^{#1}_{#2#3}}
\newcommand{\basisvecFunctime}{\boldsymbol{\basisvectimeFuncSymb}}
\newcommand{\basisvecFunctimeij}[2]{\basisvectimeFunc^{#1}_{#2}}
\newcommand{\basisvecFunctimeijk}[3]{{\basisvectimeFuncSymb}^{#1}_{#2#3}}
\newcommand{\basismatst}{\boldsymbol{\basismatstSymb}}
\newcommand{\basisvecst}{\boldsymbol{\basisvecstSymb}}
\newcommand{\operatorerrorbound}{\boldsymbol{\operatorerrorboundSymb}}
\newcommand{\basisDummy}{\boldsymbol{V}}
\newcommand{\basismatspace}{\boldsymbol{\basismatspaceSymb}}
\newcommand{\basismatspaceres}{\boldsymbol{\basismatspaceSymb}_r}
\newcommand{\basispsi}{\bm{\psi}}
\newcommand{\basisvecspace}{\boldsymbol{\basisvecspaceSymb}}
\newcommand{\basisvecspaceSubWindowArg}[3]{\boldsymbol{\basisvecspaceSymb}_{#1}^{#2,#3}}

\newcommand{\basisvecspaceres}{\boldsymbol{\basisvecspaceSymb}_r}
\newcommand{\basisvecspacei}[1]{\boldsymbol{\basisvecspaceSymb}_{#1}}
\newcommand{\basisvecspaceresi}[1]{\boldsymbol{\basisvecspaceSymb}_{r,#1}}
\newcommand{\basismatres}{\basismatspace_\resSymb}
\newcommand{\basismatrest}{{\bar \basismatspace}_\resSymb}
\newcommand{\basismatrestvec}[1]{{\bar {\boldsymbol{\basisvecspaceSymb}}_{r,#1}}}
\newcommand{\basismatrestvecFunc}[1]{{\bar
{\boldsymbol{\upphi}}_{r,#1}}}
\newcommand{\basisresi}[1]{\basismatrest^{#1}}
\newcommand{\basisres}{\boldsymbol \Pi_r}
\newcommand{\mappingresNo}{\mathcal I_r}
\newcommand{\mappingres}[2]{\mappingresNo(#1,#2)}
\newcommand{\basisresvecArg}[1]{\boldsymbol \pi_{r,#1}}
\newcommand{\basisresvecij}[2]{\basisresvecArg{\mappingres{#1}{#2}}}
\newcommand{\rfactor}{{\boldsymbol R}}
\newcommand{\basisvecres}{\basisvecspace_{\resSymb}}
\newcommand{\basisvecresst}{\bar{\basisvecspace}_{\resSymb}}
\newcommand{\basisvecressti}[1]{\basismatrestvec{#1}}
\newcommand{\basisvecresstij}[2]{\bar \basisvecspaceSymb_{\resSymb({#1},{#2})}}
\newcommand{\errorvec}{\boldsymbol \varepsilon}
\newcommand{\errorvecFunc}{\boldsymbol \upvarepsilon}
\newcommand{\errorvecFuncEntry}[1]{\upvarepsilon_{#1}}
\newcommand{\timesamplestoadd}[1]{\nrestimeind^{#1}}
\newcommand{\spacesamplestoadd}[1]{\nresspaceind^{#1}}
\newcommand{\spacetimesamplestoadd}[1]{\nressamplest^{#1}}
\newcommand{\minsamplestoadd}{\bar n_{\timeSymb,\text{min}}}
\newcommand{\weightmat}{\boldsymbol{\weightmatSymb}}
\newcommand{\weightmatwstArg}[1]{\boldsymbol{\weightmatSymb}_{\text{WST}}^{#1}}



\newcommand{\swstbasisvecTensorArg}[2]{\overrightharpoon{\bm{\pi}}^{#1}_{#2}}

\newcommand{\weightmatst}{\weightmat_{\text{ST}}}
\newcommand{\weightmatstArg}[1]{\weightmatst^{#1}}
\newcommand{\weightvecstij}[2]{\bar{\weightvecSymb}_{{#1}{#2}}}
\newcommand{\snapshots}{\boldsymbol \snapshotSymb}
\newcommand{\snapshotsSubWindowArg}[2]{\boldsymbol \snapshotSymb^{\!\!\!\!#1,#2}}

\newcommand{\snapshotsRes}{{\boldsymbol \snapshotResSymb}}
\newcommand{\snapshotsResWindowSubWindow}{\snapshotsRes^{\!\!\!k,m}_{(2)}}
%\newcommand{\snapshotmatspace}{\boldsymbol \snapshotmatspaceSymb}
%\newcommand{\snapshotmattime}{\boldsymbol \snapshotmattimeSymb}
\newcommand{\snapshotmatspace}{\tensorUnfold{1}}
\newcommand{\snapshotmattime}{\tensorUnfold{2}}
\newcommand{\snapshotmatparam}{\tensorUnfold{3}}

%\newcommand{\resn}{\res^{n}}
\newcommand{\resnst}{\resst^{n}}
\newcommand{\samplemat}{\boldsymbol \samplematSymb}
\newcommand{\samplematst}{\bar{\samplemat}}
\newcommand{\samplevec}{\boldsymbol \samplevecSymb}
\newcommand{\samplevecst}{\bar{\samplevec}}
\newcommand{\samplevecsti}[1]{\samplevecst_{#1}}
\newcommand{\resi}[1]{\res^{{#1}}}
\newcommand{\spatialSubspacei}[1]{\spatialSubspace_{#1}}
\newcommand{\temporalSubspaceFuncArg}[1]{\temporalSubspaceFunc_{#1}}
\newcommand{\temporalSubspaceArg}[1]{\temporalSubspace_{#1}}

\newcommand{\pa}[1]{\!\left(#1\right)} % Need \usepackage{amsmath}
\newcommand{\bmat}[1]{\begin{bmatrix}#1\end{bmatrix}} % Need \usepackage{amsmath}
\newcommand{\pmat}[1]{\begin{pmatrix}#1\end{pmatrix}} % Need \usepackage{amsmath}
\newcommand{\vmat}[1]{\begin{vmatrix}#1\end{vmatrix}} % Need \usepackage{amsmath}
\newcommand{\Vmat}[1]{\begin{Vmatrix}#1\end{Vmatrix}} % Need \usepackage{amsmath}
\newcommand{\Bmat}[1]{\begin{Bmatrix}#1\end{Bmatrix}} % Need \usepackage{amsmath}
\def\Abb{\mathbb{A}}
\def\Bbb{\mathbb{B}}
\def\Cbb{\mathbb{C}}
\def\Dbb{\mathbb{D}}
\def\Ebb{\mathbb{E}}
\def\Fbb{\mathbb{F}}
\def\Gbb{\mathbb{G}}
\def\Hbb{\mathbb{H}}
\def\Ibb{\mathbb{I}}
\def\Jbb{\mathbb{J}}
\def\Kbb{\mathbb{K}}
\def\Lbb{\mathbb{L}}
\def\Mbb{\mathbb{M}}
\def\Nbb{\mathbb{N}}
\def\Obb{\mathbb{O}}
\def\Pbb{\mathbb{P}}
\def\Qbb{\mathbb{Q}}
\def\Rbb{\mathbb{R}}
\def\Sbb{\mathbb{S}}
\def\Tbb{\mathbb{T}}
\def\Ubb{\mathbb{U}}
\def\Vbb{\mathbb{V}}
\def\Wbb{\mathbb{W}}
\def\Xbb{\mathbb{X}}
\def\Ybb{\mathbb{Y}}
\def\Zbb{\mathbb{Z}}
\def\onebold{\boldsymbol{1}}
\def\Abold{\boldsymbol{A}}
\def\Bbold{\boldsymbol{B}}
\def\Cbold{\boldsymbol{C}}
\def\Dbold{\boldsymbol{D}}
\def\Ebold{\boldsymbol{E}}
\def\Fbold{\boldsymbol{F}}
\def\Gbold{\boldsymbol{G}}
\def\Hbold{\boldsymbol{H}}
\def\Ibold{\boldsymbol{I}}
\def\Jbold{\boldsymbol{J}}
\def\Kbold{\boldsymbol{K}}
\def\Lbold{\boldsymbol{L}}
\def\Mbold{\boldsymbol{M}}
\def\Nbold{\boldsymbol{N}}
\def\Obold{\boldsymbol{O}}
\def\Pbold{\boldsymbol{P}}
\def\Qbold{\boldsymbol{Q}}
\def\Rbold{\boldsymbol{R}}
\def\Sbold{\boldsymbol{S}}
\def\Tbold{\boldsymbol{T}}
\def\Ubold{\boldsymbol{U}}
\def\Vbold{\boldsymbol{V}}
\def\Wbold{\boldsymbol{W}}
\def\Xbold{\boldsymbol{X}}
\def\Ybold{\boldsymbol{Y}}
\def\Zbold{\boldsymbol{Z}}
\def\abold{\boldsymbol{a}}
\def\bbold{\boldsymbol{b}}
\def\cbold{\boldsymbol{c}}
\def\dbold{\boldsymbol{d}}
\def\ebold{\boldsymbol{e}}
\def\fbold{\boldsymbol{f}}
\def\gbold{\boldsymbol{g}}
\def\hbold{\boldsymbol{h}}
\def\ibold{\boldsymbol{i}}
\def\kbold{\boldsymbol{k}}
\def\qbold{\boldsymbol{q}}
\def\pbold{\boldsymbol{p}}
\def\rbold{\boldsymbol{r}}
\def\sbold{\boldsymbol{s}}
\def\tbold{\boldsymbol{t}}
\def\ubold{\boldsymbol{u}}
\def\vbold{\boldsymbol{v}}
\def\wbold{\boldsymbol{w}}
\def\xbold{\boldsymbol{x}}
\def\ybold{\boldsymbol{y}}
\def\zbold{\boldsymbol{z}}
\def\alphabold{\boldsymbol{\alpha}}
\def\lambdabold{\boldsymbol{\lambda}}
\def\betabold{\boldsymbol{\beta}}
\def\etabold{\boldsymbol{\eta}}
\def\gammabold{\boldsymbol{\gamma}}
\def\deltabold{\boldsymbol{\delta}}
\def\mubold{\boldsymbol{\mu}}
\def\phibold{\boldsymbol{\phi}}
\def\psibold{\boldsymbol{\psi}}
%\def\phibold{\boldsymbol{\phi}}
\def\Phibold{\boldsymbol{\Phi}}
\def\Sigmabold{\boldsymbol{\Sigma}}
\def\sigmabold{\boldsymbol{\sigma}}
\def\Gammabold{\boldsymbol{\Gamma}}
\def\Omegabold{\boldsymbol{\Omega}}
\def\Thetabold{\boldsymbol{\Theta}}
\def\Lambdabold{\boldsymbol{\Lambda}}
%\def\psibold{\boldsymbol{\psi}}
\def\Psibold{\boldsymbol{\Psi}}
\def\xibold{\boldsymbol{\xi}}
%\def\xibold{\boldsymbol{\xi}}
\def\zetabold{\boldsymbol{\zeta}}
\def\zerobold{{\bf 0}}
\newtheorem{remark}{Remark}[section]
\newcommand{ \trialWSTSubspaceTensorArg}[1]{\trialSTSubspaceTensor^{#1}}
\newcommand{ \trialWSTSubspaceVectorArg}[1]{\trialSTSubspaceVector^{#1}}
\newcommand{\ST}{\mathrm{ST}}
\newcommand{\vST}{\!\mathrm{ST}}
\newcommand{ \trialSTSubspaceTensor}{\overrightharpoon{ \mathpzc{V}}_{\vST} }
\newcommand{ \trialSTSubspaceVector}{\overrightarrow { \mathpzc{V}}_{\vST} }
\newcommand{ \trialSTSubspaceColumnTensor}{\overrightharpoon{ \mathpzc{V}}_{\vST_0} }
\newcommand{ \trialSTSubspaceColumnVector}{\overrightarrow { \mathpzc{V}}_{\vST_0}  }
\newcommand{ \stbasismatTensor}{\overrightharpoon{\stbasismat}}
\newcommand{ \stbasisTensor}{\overrightharpoon{\bm{\pi}}}
\newcommand{ \stbasisVector}{\overrightharpoon{\bm{\pi}}}
\newcommand{ \stbasismatVector}{\overrightarrow{\stbasismat}}
\newcommand{\wstBasisVectorArg}[2]{\overrightarrow{\bm{\pi}}_{#1}^{#2}}
\newcommand{\wstBasisTensorArg}[2]{\overrightharpoon{\bm{\pi}}_{#1}^{#2}}
\newcommand{\solFullDiscreteTensor}{\overrightharpoon{\solFullDiscrete}}
\newcommand{\solWindowDiscreteTensorArg}[1]{\overrightharpoon{\solFullDiscrete}^{#1}}
\newcommand{\solWindowDiscreteVectorArg}[1]{\overrightarrow{\solFullDiscrete}^{#1}}

\newcommand{\solFullDiscreteVector}{\overrightarrow{\solFullDiscrete}}
\newcommand{\dumFullDiscreteTensor}{\overrightharpoon{\dumFullDiscrete}}
\newcommand{\dumWindowDiscreteTensorArg}[1]{\overrightharpoon{\dumFullDiscrete}^{#1}}
\newcommand{\dumWindowDiscreteVectorArg}[1]{\overrightarrow{\dumFullDiscrete}^{#1}}

\newcommand{\dumFullDiscreteVector}{\overrightarrow{\dumFullDiscrete}}

\newcommand{\solFullDiscreteApproxTensor}{\overrightharpoon{\solFullDiscreteApproxArg{}}}
\newcommand{\solFullDiscreteApproxVector}{\overrightarrow{\solFullDiscreteApproxArg{}}}
\newcommand{\solFullDiscreteApproxTensorArg}[1]{\solFullDiscreteApproxTensor^{#1}}
\newcommand{\solFullDiscreteApproxVectorArg}[1]{\solFullDiscreteApproxVector^{#1}}

\newcommand{\solrefWSTTensorArg}[2]{\overrightharpoon{\solFullDiscrete}_{\mathrm{ref}_{\ST}}^{#1,#2}}    
\newcommand{\solrefWSTVectorArg}[2]{\overrightarrow{\solFullDiscrete}_{\mathrm{ref}_{\ST}}^{#1,#2}}

\newcommand{\solrefSTTensor}{\overrightharpoon{\solFullDiscrete}_{\mathrm{ref}_{\ST}}}
\newcommand{\solrefSTVector}{\overrightarrow{\solFullDiscrete}_{\mathrm{ref}_{\ST}}}
\newcommand{\resFullDiscreteApproxVector}{\overrightarrow{\resFullDiscreteApproxArg{}}}
\newcommand{\resFullDiscreteApproxTensor}{\overrightharpoon{\resFullDiscreteApproxArg{}}}
\newcommand{\resFullDiscreteVector}{\overrightarrow{\resFullDiscreteArg{}}}
\newcommand{\resFullDiscreteTensor}{\overrightharpoon{\resFullDiscreteArg{}}}
\newcommand{\resWindowDiscreteTensorArg}[1]{\overrightharpoon{\resFullDiscreteArg{}}^{#1}}
\newcommand{\resWindowDiscreteVectorArg}[1]{\overrightarrow{\resFullDiscreteArg{}}^{#1}}

\newcommand{\trialSTSubspaceWinTensor}{\overrightharpoon{\mathpzc{V}}_{\vST}^k}
\newcommand{\trialSTSubspaceSubWinTensor}{\overrightharpoon{\mathpzc{V}}_{\vST}^{k,m}}

\newcommand{\trialSTSubspaceSubWinVector}{\overrightarrow{\mathpzc{V}}_{ST}^{k,m}}
\newcommand{\trialSTSubspaceColumnSubWinTensor}{\overrightharpoon{\mathpzc{V}}_{\vST_0}^{k,m}}
\newcommand{\trialSTSubspaceWinNegTensor}{\overrightharpoon{\mathpzc{V}}_{\vST}^{k-1}}
\newcommand{\trialSTSubspaceSubWinNegTensor}{\overrightharpoon{\mathpzc{V}}_{ST}^{k,m-1}}
\newcommand{\trialSTSubspaceWinVector}{\overrightarrow{\mathpzc{V}}_{\vST}^k}
\newcommand{\trialSTSubspaceWinNegVector}{\overrightarrow{\mathpzc{V}}_{ST}^{k-1}}
\newcommand{\numWindows}{n_{\mathrm{win}}}
\newcommand{\numSubWindows}{n_{\mathrm{sub}}}
\newcommand{\numSubWindowsArg}[1]{\numSubWindows^{#1}}
\newcommand{\numStepsInSubWindowArg}[2]{N_t^{#1,#2}}
\newcommand{\numSteps}{N_t}
\newcommand{\subWindowLength}{\ell_s}
\newcommand{\subWindowLengthArg}[2]{\subWindowLength^{#1,#2}}

\newcommand{\trialSTSubspaceColumnWinTensor}{\overrightharpoon{ \mathpzc{V}}_{\vST_0}^k }
\newcommand{\trialSTSubspaceColumnWinVector}{\overrightarrow{ \mathpzc{V}}_{\vST_0}^k }
\newcommand{\trialSTSubspaceColumnSubWinVector}{\overrightarrow{ \mathpzc{V}}_{ST_0}^{k,m} }
\newcommand{\vectorizeNoArg}{\mathrm{vec}}

\newcommand{\sampleMatrixWindowArg}[1]{\bm{Z}^{#1}}

\newcommand{\vectorize}[1]{\mathrm{vec}\pa{#1}}
\newcommand{\romDimSpaceTime}{n_{st}}
\newcommand{\romDimSpaceSubWindowArg}[2]{n_s^{#1,#2}}
\newcommand{\romDimResidSpaceSubWindowArg}[2]{n_{s,r }^{#1,#2}}
\newcommand{\romDimResidTimeSubWindowArg}[3]{n_{t,r}^{#1,#2,#3}}
\newcommand{\romDimTimeSubWindowArg}[2]{n_t^{#1,#2}}

\newcommand{\windowLengthArg}[1]{\windowLength^{#1}}
\newcommand{\windowLength}{\ell_w}
\newcommand{\bz}{\bm 0}
%<<<<<<< HEAD
%
%\newcommand{\airfoil}[1]{\begin{center}\noindent
%\begin{tikzpicture}\node (tiger) [anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width = 0.244\textwidth]{#1}};%
%\begin{scope}[x={(image.south east)},y={(image.north west)}]
%\node[anchor=south west,inner sep=0] (image) at (0.093,0.09) {\includegraphics[width=0.2\textwidth]{colorbar.png}};%
%\draw (0.09, 0.05) node {\footnotesize$0$};%
%\draw (0.91, 0.05) node {\footnotesize$1.1$};%
%\end{scope}
%\end{tikzpicture}
%\end{center}
%}

\newcommand{\tunderbrace}[1]{\underbrace{\let\scriptstyle\textstyle#1}}
%%% Error analysis
\newcommand{\indexMapper}{\theta}
\newcommand{\indexMapperArg}[2]{\theta(#1,#2)}
\newcommand{\windowIndexMapper}{\varphi}
\newcommand{\windowIndexMapperArg}[1]{\varphi\,\pa{#1}}
\newcommand{\subWindowIndexMapper}{\zeta}
\newcommand{\subWindowIndexMapperArg}[1]{\zeta(#1)}
\newcommand{\params}{\param}
\newcommand{\stateDumA}{\bm{\mathsl{v}}}
\newcommand{\stateDumB}{\bm{\mathsl{w}}}
\newcommand{\stateSTDumA}{\bm{\overrightarrow{\mathsl{v}}}}
\newcommand{\stateSTDumB}{\bm{\overrightarrow{\mathsl{w}}}}
\newcommand{\stateWSTDumAArg}[1]{\stateSTDumA^{#1}}

\newcommand{\approxStateST}{\overrightarrow{\tilde{\bm{\mathsl{u}}}}}
\newcommand{\approxStateWSTArg}[1]{\overrightarrow{\widetilde{\bm{\mathsl{u}}}}^{#1}}
\newcommand{\approxStateICWSTArg}[1]{{\widetilde{\bm{\mathsl{u}}}}_0^{#1}}

\newcommand{\fomStateWSTArg}[1]{\fomStateST^{#1}}
\newcommand{\fomStateICWSTArg}[1]{\fomState_0^{#1}}
\newcommand{\stateWSTDumAICArg}[1]{\stateDumA^{#1}_0}
\newcommand{\stateWSTDumBICArg}[1]{\stateDumB^{#1}_0}
\newcommand{\fomState}{{\bm{{\mathsl{u}}}}}
\newcommand{\fomStateST}{\overrightarrow{\bm{{\mathsl{u}}}}}
\newcommand{\fomStateStarWSTArg}[1]{\fomStateST_*^{#1}}
\newcommand{\fomStateProjectWSTArg}[1]{\fomStateST_{\ell^2}^{#1}}
\newcommand{\fomStateProjectICWSTArg}[1]{\fomState_{\ell^2,0}^{#1}}
\newcommand{\errorWST}{\overrightarrow{\bm{{\mathsl{e}}}}}
\newcommand{\errorWSTArg}[1]{\errorWST^{#1}}
\newcommand{\errorICWSTArg}[1]{\errorWST_0^{#1}}

\newcommand{\stateICWSTDumAArg}[1]{\stateSTDumA_{0}^{#1}} 
\newcommand{\AWSTArg}[1]{\mathbf{E}^{#1}}
\newcommand{\BWSTArg}[1]{\mathbf{F}^{#1}}
\newcommand{\AICWSTArg}[1]{\mathbf{E}_0^{#1}}
\newcommand{\BICWSTArg}[1]{\mathbf{F}_0^{#1}}
\newcommand{\stateWSTDumBArg}[1]{\stateSTDumB^{#1}}
\newcommand{\tST}{\overrightarrow{\boldsymbol t}}
\newcommand{\tWSTArg}[1]{\tST^{#1}}

\newcommand{\lipschitzVelocity}{\kappa_f}
\newcommand{\lipschitzVelocityST}{\overrightarrow{\kappa}_{f}}
\newcommand{\fluxST}{\overrightarrow{\flux}}
\newcommand{\fluxWSTArg}[1]{\overrightarrow{\flux}^{#1}}
\newcommand{\fluxICWSTArg}[1]{\overrightarrow{\flux}_0^{#1}}

\newcommand{\sigmaMaxArg}[1]{\sigma_{\mathrm{max}}\pa{#1}}
\newcommand{\sigmaMaxArgSmall}[1]{\sigma_{\mathrm{max}}(#1)}
\newcommand{\sigmaMinArg}[1]{\sigma_{\mathrm{min}}\pa{#1}}
\newcommand{\sigmaMinArgSmall}[1]{\sigma_{\mathrm{min}}(#1)}
\newcommand{\constantAWSTArg}[1]{C_1^{#1}}
\newcommand{\constantBWSTArg}[1]{C_2^{#1}}
\newcommand{\T}{\!\scalebox{0.8}{$T$}}
%=======
\newcommand{\airfoilbar}[2]{%
\begin{tikzpicture}
\begin{scope}[execute at begin node=$, execute at end node=$]
\node (tiger) [anchor=south west,inner sep=0,label=below:#2] (image) at (0,0){\includegraphics[width = 0.2415\textwidth,frame]{#1}};
\end{scope}
\node[anchor=south west,inner sep=0] (image) at (0.42,0.5) {\includegraphics[width=0.19\textwidth,frame]{colorbar.png}};
\draw (0.425, 0.3) node {\footnotesize{$0$}};
\draw (3.7, 0.3) node {\footnotesize{$1.1$}};
\end{tikzpicture}}

\newcommand{\airfoil}[2]{%
\begin{tikzpicture}
\begin{scope}[execute at begin node=$, execute at end node=$]
\node (tiger) [anchor=south west,inner sep=0,label=below:#2] (image) at (0,0){\includegraphics[width = 0.2415\textwidth,frame]{#1}};
\end{scope}
\end{tikzpicture}
}
\newcommand\CircledImage[1]{%
\tikz\path[fill overzoom image={#1}, draw=blue, line width=2mm]circle[radius=0.5\linewidth];%
}

% \newcommand{\samplemesh}[2]{%
% \begin{tikzpicture}
% \node (tiger) [anchor=south west,inner sep=0] (image) at (0,0){\includegraphics[width = 0.28\textwidth,frame]{#1}};
% \draw[black, thick] (2.88,2.41) -- (2.67,1.2);     
% \draw[black, thick] (3.03,2.52) -- (4.236,2.303);  
% \node[circle,draw, text=white,minimum size=3cm,
%           path picture={
%               \node at (path picture bounding box.center){
%                   \includegraphics[width=3cm]{#2}
%               };
%           }] at (4.12,0.8){};
% \draw[white, thick] (2.99,2.42) circle (3pt)
% \end{tikzpicture}}

\newcommand{\samplemesh}[2]{%
\begin{tikzpicture}
\node (tiger) [anchor=south west,inner sep=0] (image) at (0,0){\includegraphics[width = 0.22\textwidth,frame]{#1}};
\draw[black, line width=2.4pt] (2.41,1.83) -- (3.05,1); 
\draw[black, line width=2.4pt] (2.35,1.899) circle (3pt);
\draw[white, line width=1.2pt] (2.41,1.83) -- (3.05,1); 
\draw[white, line width=1.2pt] (2.35,1.899) circle (3pt);
\node[circle,draw,line width=0.6pt, text=white,minimum size=2cm,
          path picture={
              \node at (path picture bounding box.center){
                  \includegraphics[width=2cm]{#2}
              };
          }] at (3.2,0.8){};
\end{tikzpicture}}

 

%>>>>>>> bce253ce354539335990e349c96a5c6b87f363a9

%% basis fig 
\newcommand{\h}{\mkern-11mu}
\newcommand{\hb}{\mkern-5mu}
\newcommand{\pareto}[1]{\includegraphics[height=0.217\textwidth,valign=t]{#1}}
%248
\newcommand{\legend}[1]{\includegraphics[height=0.186\textwidth,valign=t]{#1}}


==> introOutline.tex <==

Literature Review of Methods: their pros and their cons
\begin{itemize}

        \item Galerkin (Willcox et. al, Carlberg et. al)
        \begin{itemize}
            \item {\color{red}Galerkin ROMS are unstable for long time intervals}
        \end{itemize}
        \item Least Squares Petrov--Galerkin (Bui-Thanh et. al, Carlberg et.al)
        \begin{itemize}
            \item {\color{orange}dependent on time step}
            \item decreasing time step does not necessarily decrease the error for LSPG ROM
        \end{itemize}
        \item Windowed Least Squares method (Parish et. al)
        \begin{itemize}
            \item Accuracy of ROM is independent of the time step/time discretization methods
        \end{itemize}
        \item Space--Time Least Squares Petrov--Galerkin (choi et. al)
            \begin{itemize}
                \item Performs spatial AND temporal reduction
                \item performs aggressive reduction of the time domain
                \item a priori error bound in terms of the best space--time approximation error
                \item {\color{red} Performs projection over the entire time interval of interest}
                \item {\color{red} Large computational cost because it destroys the natural block lower triangular structure of the original space--time problem. }
                \item {\color{red} time-marching solvers have a complexity that is linear in the time dimension but this approach requires dense space--time solvers whose complexity is cubic in the time dimension.}
            \end{itemize}
        \item time parallel methods 
            \begin{itemize} 
                \item Enable dynamical-system simulations to be paralleled in the temporal domain
                \item well suited fore ROMS
                \item {\color{red} does not reduce temporal dimensionality. It increases total computational cost of simulation as measured in core-hours}
            \end{itemize}
        \item forecasting approach
            \begin{itemize}
                \item employs time-domain data generated during offline stage of model reduction produce accurate forecasts of the solution during online ROM simulations via gappy POD.
                \item generates accurate initial guesses for newton solver
                \item coarse propagator to accelerate convergence of time-parallel methods
                \item reduces computational cost incurred by time integration by reducing newton iterations 
                \item {\color{red} does not reduce the temporal dimension of the ROM}
            \end{itemize}
        \item space--time ROMS using reduced basis
            \begin{itemize}
                \item reduces temporal dimension of the model using projections with low dimensional space--time basis.
                \item removes spurious temporal modes from the state space
                \item equipped with errors bounds grow linearly rather than exponentially throughout entire simulation time
                \item {\color{red} requires space--time finite element discretization}
                \item {\color{red} do not provide for complexity reduction such as hyper-reduction }
                \item {\color{red} computes only single space--time basis vector per training simulation limiting the dimensionality and accuracy of the resulting space--time ROM}
            \end{itemize}
        \item Spatial Local reduced-order model (Amsallem et. al)
            \begin{itemize}
                \item provides better nonlinear ROM approximations by using local reduced order basis instead of the global reduced order basis.
                \item uses local reduced order basis that are tailored for the purpose of capturing only the local behavior of a nonlinear or parametric system at a given point of the state space.
                \item uses POD to create the local basis 
                \item local ROBS are not linked a priori neither to a time-domain not ro a space-domain partition
                \item built using unsupervised learning algorithm that clusters snapshots without any a priori assumption
                \item does not require any projections when switching from one local ROB to another
                \item hyper reduction can be used
                \item Shows that this technique more accurate and computationally more efficient and superior to the standard global counterpart
            \end{itemize}
        \item Windowed Least-Squares Petrov Galerkin Technique
        \begin{itemize}
            \item solver is fully space--time coupled within a window, but is sequential across windows. The complexity is linear as a result in the number of time windows, and cubic int he time dimension within the windows 
            \item generalization of both ST-LSPG and WST-LSPG
            \item proposes a variety of methods for constructing the space--time basis using tensor decompositions performed over each window (as a function of sub windows)
            \item Error analysis shows that errors accumulate exponentially across time windows
            \item due to the "superior" complexity scaling of WST-LSPG relative to ST-LSPG (linear cost in number of time windows), WST-LSPG nearly always outperforms ST-LSPG.
            \item better behavior than sequential ROMS, where error accumulation is exponential across time steps
            \item {\color{red} Kevin says that we are no longer bounded by the best approximation error as in ST-LSPG due to the sequential approximations across time windows}
        \end{itemize}

\end{itemize}


==> nomenclature.tex <==


% % \setlength{\nomlabelwidth}{1.5cm}

% %----------------------------------------------------------
% % States
% %----------------------------------------------------------
% \nomenclature[U]{$u$}{scalar quantity for state}
% \nomenclature[U]{$\solFullDiscreteArg{n}$}{\EP{what are your thoughts for $\mathbf{u}^n$ for the discretized in space discretized in time state, opposed to $\bm{u}^n$? Both are fine though. I think we should avoid $\bm{u}(t^n)$, as this reads as if we are evaluating a continuous in time function at the time instance $t^n$. Same comment holds for the residual)}\\
% \YS{I agree with your comment about $\bm{u}(t^n)$. Let me think more about $\bm{u}^n$ vs. $\mathbf{u}^n$. Kevin's notations in the ST-LSPG paper are so confusing. update: lets use $\solFullDiscrete$? ( $\bm{u}^n$ vs. $\mathbf{u}^n$ vs. $\solFullDiscrete^n$ ) I don't really like nonslanted/non italicized math symbols.} \EP{Sounds great to me, I like it!}}
% \nomenclature[U]{$\state(t^n)$}{discrete in space continuous in time state evaluated at $t^n$}
% \nomenclature[U]{$\snapshots$}{$\bm{g}(\bm{\state})$, unrolled form discrete space and time states}
% \nomenclature[U]{$\solTimeContinuous$}{discretized in space continuous in time states}

% %----------------------------------------------------------
% % Residuals
% %----------------------------------------------------------
% \nomenclature[R]{$\resTimeContinuous$}{discretized in space continuous in time residual }
% \nomenclature[R]{$r$}{scalar quantity for residual}
% \nomenclature[R]{$\bm{r}(t^n)$}{discrete in space continuous in time residual evaluated at $t^n$}
% \nomenclature[R]{$\resFullDiscreteArg{n}$}{vector quantity for discretized in space discretized in time residual at time index $n$}
% \nomenclature[R]{$\snapshotsRes$}{$\bm{g}(\bm{r})$, unrolled form discrete space and time residual}
% \nomenclature[R]{$\fluxFullDiscreteArg$}{discrete in time and space flux or velocity}

% %----------------------------------------------------------
% % Dummy Variables
% %----------------------------------------------------------
% \nomenclature[W]{$\bm{X}_y$}{$\bm{g}(\bm{y})$, unrolled form discrete space and time dummy variable}
% \nomenclature[W]{\bm{w}}{generic, dummy variable for variables that are same size as the states and residuals}
% \nomenclature[W]{$\dummyFullDiscrete$}{generic, dummy variable for trial basis}
% \nomenclature[W]{$\dummyBasisDiscrete$}{trial basis}
% \nomenclature[X]{$\tensor$}{3-way tensor}
% \nomenclature[X]{$\tensorSub{y}$}{3-way tensor of the `unrolled' function of $y$}

% \nomenclature[S]{$\trialSSubspace$}{spatial trial subspace}
% \nomenclature[S]{$\testSSubspace$}{spatial test subspace}
% \nomenclature[S]{$\trialSTSubspace$}{spatial-temporal trial subspace}
% \nomenclature[S]{$\testSTSubspace$}{spatial-temporal test subspace}


